Scalable Group Choreography via Variational Phase Manifold Learning

Generating group dance motion from the music is a challenging task with several industrial applications. Although several methods have been proposed to tackle this problem, most of them prioritize optimizing the fidelity in dancing movement, constrained by predetermined dancer counts in datasets. This limitation impedes adaptability to real-world applications. Our study addresses the scalability problem in group choreography while preserving naturalness and synchronization. In particular, we propose a phase-based variational generative model for group dance generation on learning a generative manifold. Our method achieves high-fidelity group dance motion and enables the generation with an unlimited number of dancers while consuming only a minimal and constant amount of memory. The intensive experiments on two public datasets show that our proposed method outperforms recent state-of-the-art approaches by a large margin and is scalable to a great number of dancers beyond the training data.

==> 4_method_old.tex <==
\section{Methodology}

\subsection{Task Definition}
Given an input music sequence $\{a_1, a_t, ...,a_T\}$ with $t = \{1,..., T\}$ indicates the index of the music frames, our goal is to generate the group motion sequences of $N$ dancers: $\{x^1_1,..., x^1_T; ...;x^N_1,...,x^N_T\}$ where $x^n_t$ is the pose of $n$-th dancer at frame $t$. 
We represent dances as sequences of poses in the 24-joint of the SMPL model~\cite{SMPL:2015}, using the 6D continuous rotation~\cite{zhou2019rotation_6d} for every joint, along with a single 3D root translation.
Previous group dance methods~\cite{le2023music}, which generate the whole group at once, cannot deal with the increasing number of dancers and can only create group sequence up to a pre-defined number of dancers, due to the complexity of architecture. In contrast, we aim to generate group dance with an unlimited number of dancers.


% \begin{figure*}[ht]
%     \centering
%     \includegraphics[width=1\textwidth, keepaspectratio=true]{images/PhaseVAE.png}
%     \vspace{-3ex}
%     \caption{Phase Variational Autoencoder}
%     \vspace{-1ex}
%     \label{fig:phasevae_single}
% \end{figure*}
\begin{figure*}[ht]
    \centering
    \includegraphics[width=1\textwidth, keepaspectratio=true]{images/CVAE_train.png}
    \vspace{-3ex}
    \caption{\textbf{We should re-organize the Figure, keep 1 or 2 figure to illustrate our contribution} Group-constraint Music-conditional Phase VAE}
    \vspace{-1ex}
    \label{fig:CVAE}
\end{figure*}

\subsection{Learning Phase Representation for Motion}
\label{sec:pae}
Our goal is to learn a continuous manifold such that the motion can be  generated by sampling from this learned manifold. We assume that although different dancers within the same group may present visually distinctive movements, their motions' properties such as timing, periodicity or temporal alignment are intrinsically similar. Drawing inspiration from DeepPhase~\cite{starke2022deepphase}, an Autoencoder architecture that can learn a well-structured phase manifold from the unstructured character movements, we aim to learn a generative phase representation for each whole group in order to synthesize their motion limitlessly. The latent phase manifold can well describe key information of the motion such as its timing, local periodicity, and transition.  Given an input motion curve $x$, we first use an encoder to encode it into a lower dimensional embedding space,
% Firstly, we utilize a 1D Temporal Convolutional Encoder to encode the motion sequence $x$ into a lower dimensional embedding space, followed by two separate Conv1D layers to transform into mean and variance of the VAE model~\cite{kingma2013vae}.
\begin{equation}
    \mathbf{L} = E(x)
\end{equation}
where $\mathbf{L} \in \mathbb{R}^{D \times T}$ with $D$ is the number of latent channels, that is, the number of desired phase channels to be extracted from the motion. 
To enforce learning periodicity of the motion, we parameterize each latent curve in $\mathbf{L}$ using a sinusoidal function with amplitude ($A$), frequency ($F$), offset ($B$) and phase shift ($S$) parameters~\cite{starke2022deepphase}. To do so, we first apply differentiable Fast Fourier Transform (FFT) to each channel of the latent curve $\mathbf{L}$ and create the zero-indexed matrix of Fourier coefficients as $\mathbf{c}=FFT(\mathbf{L})$ with $\mathbf{c} \in \mathbb{C}^{D \times K+1}$, $K =\lfloor \frac{T}{2}\rfloor$.

The per channel power spectrum $\mathbf{p} \in \mathbb{R}^{D \times K+1}$ is s $\mathbf{p}_{i,j} = \frac{2}{N}|\mathbf{c}_{i,j}|^2$, where $i$ is the channel index and $j$ is the index for the frequency bands. The parameters of the sinusoidal function are then computed as follows:
\begin{equation}
    \mathbf{A}_i = \sqrt{\frac{2}{T}\sum_{j=1}^K \mathbf{p}_{i,j}}, \quad
    \mathbf{F}_i = \frac{\sum_{j=1}^K \mathbf{f}_j \cdot \mathbf{p}_{i,j}}{ \sum_{j=1}^K \mathbf{p}_{i,j}}, \quad 
    \mathbf{B}_i = \frac{\mathbf{c}_{i,0}}{T},
\end{equation}
where $\mathbf{f} = (0, \frac{1}{T},\dots,\frac{K}{T})$ is the frequencies vector.

We also use a fully-connected (FC) layer to predict the phase shift $\mathbf{S}$, which is formulated as:
\begin{equation}
    (s_y, s_x)  = FC(\mathbf{L}_i), \quad \mathbf{S}_i = \arctan(s_y,s_x),
\end{equation}
Subsequently,  those parameters $$(A,F,B,S)$$ are used to calculate a parametric latent space consisting of multiple periodic curves to represent each intrinsic property of the motion by:
\begin{equation}
    \hat{\mathbf{L}} = \mathbf{A} \cdot \sin (2\pi \cdot (\mathbf{F}\cdot\mathcal{T} - \mathbf{S})) + \mathbf{B}
\end{equation}
where $\mathcal{T}$ is a known time window series obtained by evenly spacing the timesteps. Finally, a decoder is utilized to reconstruct the original input signals from the set of parametric latent curves: \begin{equation}
\hat{x} = D(\hat{\mathbf{L}})
\end{equation}


% \begin{figure*}[ht]
%     \centering
%     \includegraphics[width=1\textwidth, keepaspectratio=true]{images/CVAE_transformer.png}
%     \vspace{-3ex}
%     \caption{Group-constraint Music-conditional Phase VAE}
%     \vspace{-1ex}
%     \label{fig:CVAE}
% \end{figure*}


\subsection{Music-Conditioned VAE}
To facilitate motion generation from music, we adopt a conditional VAE~\cite{sohn2015cvae} framework whose goal is to learn a joint latent distribution between two modalities (motion and music). Specifically, the model contains three main networks: an encoder $\mathcal{E}$ to capture the approximate posterior distribution conditioned on both motion and music $q_\phi(z|x,a)$, a prior network $\mathcal{P}$ to learn the conditional prior given only the music $p_\theta(z|a)$ , and a decoder $\mathcal{D}$ to learn to reconstruct the data from the 
latent distribution $p_\theta(x|z,a)$. Furthermore, we design these networks based on Transformer architecture~\cite{vaswani2017attention} to effectively capture long-range dependencies and holistic context in sequence modeling. 


\textbf{Encoder.} The Encoder takes both motion and music sequences as input, and produces a distribution over possible latent variables $z$ capturing the cross-modal relationship between them. Mathematically, it is parameterized by a Gaussian distribution:
\begin{equation}
    q_\phi(z|x,a) = \mathcal{N}(z; \mu_\phi(x,a), \Sigma_\phi(x,a))
\end{equation}
where $\mu_\phi$ and $\Sigma_\phi$ are the predicted mean and variance by the Transform network given its corresponding inputs. We implement the Encoder following the Transformer Decoder architecture where the Cross-Attention mechanism~\cite{vaswani2017attention} is utilized to learn the relationship between the motion and the music. In particular, the input motion is treated as the query while the music is projected into the corresponding key and value. We then calculate their cross-attention as follows:
\begin{align}
    \label{eq:cross_attention}
    {Q}_{e} = W^Q_e x, \quad {K}_{e} = W^K_e a, \quad {V}_{e} = W^V_e a, \\
    \text{CrossAtt}(Q_e, K_e, V_e) = \text{softmax}\left(\frac{Q_e K_e^\top}{\sqrt{d_k}} \right) V_e,
\end{align}
where ${W}^{Q}_e, {W}^{K}_e \in \mathbb{R}^{d \times d_k}$ and ${W}^{V} \in \mathbb{R}^{d \times d_v}$ are learnable projection matrices to map the inputs into query, key, and value, respectively. In addition, we also append two extra learnable tokens $\mu_{token}$ and $\Sigma_{token}$ to the input motion sequence to represent the input signals for the mean and variance. The latent distribution parameters $\mu$ and $\Sigma$ are obtained by taking the outputs of the encoder that correspond to the two extra input tokens.
By doing this way instead of conventional temporal pooling the sequence to get a representative vector, the model will be able to learn a more expressive latent space as the mean and variance tokens are calculated by effectively applying attention across the sequence with global receptive fields, which is also less susceptible to noisy frames thanks to the nature of attention mechanism.

\textbf{Prior Network.} Since the motion is mostly inaccessible at test time (only the music is available), we need to learn a prior to match the posterior distribution of motion in order to draw samples from.  Instead of imposing the prior distribution to be standard normal (i.e. $\mathcal{N}(0,I)$ as in conventional VAE~\cite{kingma2013vae}, we relate it to the music condition. Therefore, our conditional prior is defined as:
\begin{equation}
p_\theta(z|a) = \mathcal{N}(z;\mu_\theta(a), \Sigma_\theta(a))
\end{equation}  
where a Transformer model is used to encode the input conditioning music sequence and predict the corresponding $\mu_\theta$ and $\Sigma_\theta$. We implement the Prior network similarly to the Encoder, however, here we use self-attention mechanism~\cite{vaswani2017attention} to capture the global music context. Intuitively, each latent variable $z$ is expected to represent (almost) every possible dance motion $x$ conforming to the music context $a$. Therefore, it should have different distributions given different music $a$. For example, the dance distribution conditioned on "pop" music should be different from the distribution conditioned on "hip hop". Learning the conditional prior significantly improves the ability of the CVAE to generalize to diverse types of music and motion.
 
Accordingly, from the encoded latent distribution,  we sample a latent vector $z \in \mathbb{R}^{d}$ using the reparameterization trick~\cite{kingma2013vae}. This latent vector is then passed through the decoder to generate natural output motion sequences following data distribution.

\textbf{Decoder.} Conditioned on the latent vector $z$, the Decoder aims to produce human motion for a given music duration in one go (i.e., non-autoregressive). It is a Transformer decoder that takes a single latent vector $z$, the music features $a$ as inputs, as well as an initialized hidden sequence $h$ to start decoding for attention to be applicable.
\begin{align}
    p_\theta(x|z,a) = \mathcal{D}(z,a,h), \\
    \mathcal{D}(z,a,h) = \text{CrossAtt}(h, [z;a], [z;a])
\end{align}
where $[z;a]$ denotes the concatenation between $z$ and $a$, and the $\text{CrossAtt}$ is calculated similarly to Eq.~\ref{eq:cross_attention}. Here, we also utilize cross-attention model where we consider the combined sequence of latent vector and music features as key and value, and the initialized sequence as the query. There are several design choices to initialize the hidden query sequence $h$, such as constructing it as a sinusoidal positional encoding sequence with duration $T$ as in~\cite{} or leveraging the encoded output sequence of the Encoder/Prior network. However, in our experiment, we observed that these techniques usually result in unstable training and inconsistent output, as the initialized sequence is quite generic and usually contains less meaningful information for the decoder. 

To alleviate this issue, we propose to use the Phase information to initialize the hidden sequence. Specifically, we impose the PAE network (Section~\ref{sec:pae}) inside the CVAE model, where we apply a differentiable FFT layer to extract the hidden output sequence of the Encoder/Prior network into frequency-domain parameters. The latent signals are then reconstructed from those parameters by using a set of sinusoidal functions.This operation can be (roughly) viewed as using a "quantization" layer to enforce the network to learn to embed the motion features in the frequency domain, which is more useful in representing different aspects of human motion (such as timing or periodicity).


\textbf{Training.} During training, we consider the following variational lower bound to mainly train our VAE model:
\begin{equation}
\log p_\theta(x|a) \geq \mathbb{E}_{q_\phi} \left[ \log p_\theta(x|z,a) \right] - D_{\text{KL}}(q_\phi(z|x,a) \Vert p_\theta(z|a))
\end{equation}
The first term measures reconstruction error given the decoder output, while
the second term penalizes the KL-divergence $D_{\text{KL}}$ between the posterior and the prior distribution to enforce them to be close to each other. We further increase the group consistency by imposing KL-divergence between different dancer within the same group. This is used to make sure every dancer is embedded into a single unified manifold that represents the group they belong to. For testing, we can efficiently generate motions for unlimited dancers by indefinitely drawing samples from this continuous unified group manifold. We note that for inference, we only need to process the Prior network once to obtain the latent distribution. To generate a new motion, we efficiently sample from this latent (Gaussian) distribution and use the Decoder to decode it back to the motion space. It is much more efficient and has higher scalability than previous approaches~\cite{le2023controllableGCD,le2023music} which is limited by the number of dancers to be processed simultaneously by the entire network.





% \begin{figure*}[ht]
%     \centering
%     \includegraphics[width=1\textwidth, keepaspectratio=true]{images/PC_VAE_&_Scene_refinement.png}
%     \vspace{-3ex}
%     \caption{Phase-conditioned Trajectory Generation}
%     \vspace{-1ex}
%     \label{fig:trajectory_refinement}
% \end{figure*}
